Unconditionally successful quantum Time-Marching algorithm via LCU for nonlinear Burgers equation

Most recently proposed quantum algorithms for solving linear and nonlinear partial differential equations rely on non-unitary operations. These operations are typically implemented probabilistically, requiring postselection and thus increasing the computational cost. We show that quantum lattice gas algorithms enable unconditionally successful quantum simulation of nonlinearities, yielding, to our knowledge, the first quantum algorithm for Burgers equation whose time steps can be concatenated without probabilistic failure. The key idea is to exploit the correspondence between the stochasticity of quantum measurement in the linear combination of unitaries framework and the intrinsic randomness of the classical lattice gas algorithm. In doing so, we identify general properties that characterize probabilistic classical algorithms amenable to this time-marching formulation, and illustrate the approach with an additional application.

==> Fig3code.tex <==
\begin{figure}[ht]
    \centering
    \scalebox{0.85}{
    \begin{tikzpicture}
        \def\l{0.5}
        
        \newcommand{\drawlattice}{
        \foreach \j in {0,1.5,3}{
        \foreach \i in {0,1,2,3,4,5}
                {
                \draw[fill=white] (\i, \j) circle (3pt);
                }
            }
        }
        
        \newcommand{\drawarrows}[3]{
        \foreach \ang in {#3}{
        \draw[-stealth, black, thick] 
        ({#1 + 0.1 * cos(\ang)}, #2) -- ({#1 + \l*cos(\ang)},#2);}}
        \newcommand{\drawrest}[2]{
        \draw[fill=black] (#1, #2) circle (3pt);
        }
        
        \drawlattice
        \drawarrows{0}{3}{0,180}
        \drawarrows{1}{3}{0}
        \drawarrows{3}{3}{180}
        \drawarrows{4}{3}{0}
        \filldraw[black] (0, 2.5) node[anchor=center]{$[11]$};
        \filldraw[black] (1, 2.5) node[anchor=center]{$[01]$};
        \filldraw[black] (2, 2.5) node[anchor=center]{$[00]$};
        \filldraw[black] (3, 2.5) node[anchor=center]{$[10]$};
        \filldraw[black] (4, 2.5) node[anchor=center]{$[01]$};
        \filldraw[black] (5, 2.5) node[anchor=center]{$[00]$};
        \draw[gray, thick] (-3.5,2) -- (5.5,2);
        \drawarrows{0}{1.5}{0,180}
        \drawarrows{1}{1.5}{0}
        \drawarrows{3}{1.5}{0}
        \drawarrows{4}{1.5}{180}
        \filldraw[black] (0, 1) node[anchor=center]{$[11]$};
        \filldraw[black] (1, 1) node[anchor=center]{$[01]$};
        \filldraw[black] (2, 1) node[anchor=center]{$[00]$};
        \filldraw[black] (3, 1) node[anchor=center]{$[01]$};
        \filldraw[black] (4, 1) node[anchor=center]{$[10]$};
        \filldraw[black] (5, 1) node[anchor=center]{$[00]$};
        \draw[gray, thick] (-3.5,0.5) -- (5.5,0.5);
        
        \drawarrows{1}{0}{0}
        \drawarrows{2}{0}{0}
        \drawarrows{3}{0}{180}
        \drawarrows{4}{0}{0}
        \drawarrows{5}{0}{180}
        \filldraw[black] (0, -0.5) node[anchor=center]{$[00]$};
        \filldraw[black] (1, -0.5) node[anchor=center]{$[01]$};
        \filldraw[black] (2, -0.5) node[anchor=center]{$[01]$};
        \filldraw[black] (3, -0.5) node[anchor=center]{$[10]$};
        \filldraw[black] (4, -0.5) node[anchor=center]{$[01]$};
        \filldraw[black] (5, -0.5) node[anchor=center]{$[10]$};

        \filldraw[black] (-2, 4) node[anchor=center]{$x$};
        \filldraw[black] (0, 4) node[anchor=center]{$0$};
        \filldraw[black] (1, 4) node[anchor=center]{$1$};
        \filldraw[black] (2, 4) node[anchor=center]{$2$};
        \filldraw[black] (3, 4) node[anchor=center]{$3$};
        \filldraw[black] (4, 4) node[anchor=center]{$4$};
        \filldraw[black] (5, 4) node[anchor=center]{$5$};
        
        \filldraw[black] (-2, 2.75) node[anchor=center]{Before collision};
        \filldraw[black] (-2, 1.25) node[anchor=center]{After collision};
        \filldraw[black] (-2, -0.25) node[anchor=center]{After streaming};
    \end{tikzpicture}
    }
    \caption{Example of classical evolution \cite{boghosian2019cellular}. The collision takes place  at $x=1,3,4$, with different random extractions for $\alpha$. All the other cells are not affected by the collision. The streaming takes place according to respective velocities with continuous boundary conditions.}
    \label{fig:boghosian}
\end{figure}
